Token Fusion: Bridging the Gap between Token Pruning and Token Merging

Vision Transformers (ViTs) have emerged as powerful backbones in computer vision, outperforming many traditional CNNs. However, their computational overhead, largely attributed to the self-attention mechanism, makes deployment on resource-constrained edge devices challenging. Multiple solutions rely on token pruning or token merging. In this paper, we introduce "Token Fusion" (ToFu), a method that amalgamates the benefits of both token pruning and token merging. Token pruning proves advantageous when the model exhibits sensitivity to input interpolations, while token merging is effective when the model manifests close to linear responses to inputs. We combine this to propose a new scheme called Token Fusion. Moreover, we tackle the limitations of average merging, which doesn't preserve the intrinsic feature norm, resulting in distributional shifts. To mitigate this, we introduce MLERP merging, a variant of the SLERP technique, tailored to merge multiple tokens while maintaining the norm distribution. ToFu is versatile, applicable to ViTs with or without additional training. Our empirical evaluations indicate that ToFu establishes new benchmarks in both classification and image generation tasks concerning computational efficiency and model accuracy.

==> manuscripts/legacy.tex <==

\subsection{From Local to Highway $(D)$}
\label{sec:D}
The objective of \( D \) is to distribute the local features into the full token features by positioning the merged tokens back to their source indexes. An efficient approach is to maintain \( I \in \mathbb{R}^{N} \), a local path index for each token in the full path. We initiate \( I \) as \( I = \{i \mid 0 \leq i < N\} \), which is a range from 0 to the length of the full token. With $\text{idx}_{\text{src}}, \text{idx}_{\text{dst}}$ from ``Reduce" operation, we update $I$ to reflect where in local path the token is pointing to. 
For a specific local feature \( \mathbf{F}_{local} \), which can either be \( \text{ATTN}(\mathbf{X}_{local}) \) or \( \text{MLP}(\mathbf{X}_{local}) \), \( I \) aids in distributing \( \mathbf{F}_{local} \) into the full structure. The specifics of \( D \) are described in Algorithm~\ref{algo:2}.

\begin{algorithm}
\caption{Token Highway \( D(X) \)}
\begin{algorithmic}[1]
\State \textbf{Input:} \( \mathbf{F}_{local}, I, \text{idx}_{\text{src}}, \text{idx}_{\text{dst}} \)
\State \textbf{Output:} \( \mathbf{F}_{full}, I \)
\State \( I \leftarrow I.\text{scatter}(\text{dim=}1, \text{index=}\text{idx}_{\text{src}}, \text{src=}\text{idx}_{\text{dst}}) \)
\State \( \mathbf{F}_{empty} \leftarrow \text{empty tensor of size } \mathbf{F}_{full} \)
\State \( \mathbf{F}_{full} \leftarrow \mathbf{F}_{empty}.\text{scatter}(\mathbf{F}_{local}, \text{index}=I) \)
\end{algorithmic}
\label{algo:2}
% \caption{Algorithm details for the distribute function in Token Highway.}
\end{algorithm}


\paragraph{Magnitude Based Masking (MBM)} Highway path is  
\begin{equation}
    \mathbf{X}_{full}' = \mathbf{X}_{full} + D(\mathbf{F}_{local}).
\end{equation}
Since \( D \) approximates the full path with the copying operation, some tokens may not be accurate. We introduce an additional operation to refine this approximation. Although it's conceivable to learn an auxiliary network to enhance \( D \) for better approximation, we avoid this to ensure our algorithm remains versatile and efficient. Instead, we tweak \( D(\mathbf{F}_{local}) \) to influence \( \mathbf{X}_{full}' \) less if the preceding full feature \( \mathbf{X}_{full} \) has a larger value. Specifically, we let a mask, 
\begin{align}
    \mathbf{M}[i, j] &=
\begin{cases}
0 & \text{if } |\mathbf{X}_{full}[i, j]| \geq t  \text{ \& } i \in \left(\text{idx}_{src} \cup \text{idx}_{dst}\right) \\
1 & \text{otherwise }
\end{cases} \nonumber \\
    \mathbf{X}_{full}' &= \mathbf{X}_{full} + \mathbf{M} \odot D(\mathbf{F}_{local}).
\end{align} 
This formula nullifies elements of \( D(\mathbf{F}_{local}) \) if the token is affected by \( R \) and the magnitude of the previous token is above the threshold \( t \). This supplementary approximation step, relying on prior tokens, further enhances performance.




\subsection{Multiple Modules with Stacked Operation}

When incorporating multiple Token Highway modules in a model, a straightforward approach might suggest stacking them consecutively, incrementing \( r \) with each layer.
% \begin{align}
%     \text{Layer 1}\nonumber\\
%     &\mathbf{X}_1^* = \mathbf{X}_1 + D_A^1(\text{ATTN}(R_A^1(\mathbf{X}_1))) \\
%     &\mathbf{Y}_1 = \mathbf{X}_1^* + D_M^1(\text{MLP}(R_M^1(\mathbf{X}_1^*))) \nonumber\\
%     \text{Layer 2}\nonumber\\
%     &\mathbf{X}_2^* = \mathbf{Y}_1 + D_A^2(\text{ATTN}(R_A^2(\mathbf{Y}_1))) \\
%     &\mathbf{Y}_2 = \mathbf{X}_2^* + D_M^2(\text{MLP}(R_M^2(\mathbf{X}_2^*))).\nonumber
% \end{align}
\begin{align}
    &\mathbf{X}_1^* = \mathbf{X}_1 + D_A(\text{ATTN}(R_A(\mathbf{X}))) \\
    &\mathbf{Y}_1 = \mathbf{X}_1^* + D_M(\text{MLP}(R_M(\mathbf{X}^*)))
\end{align}
However, such a direct approach may yield suboptimal outcomes. The reason lies in the fact that \( R \) and \( D \) operations generate token duplicates. To enhance efficiency, successive layers should curtail the propagation of these duplicates by utilizing the same \( R \) operation from preceding layers. This can be achieved by compositing the ``Distribute" and ``Reduce" operations. To illustrate, consider the workings of a two-layer setup:
\begin{align}
    \mathbf{X}_1^* &= \mathbf{X}_1 + D_A(\text{ATTN}(R_A(\mathbf{X}_1))) \\
    \mathbf{Y}_2 &= \mathbf{X}_2^* + D_A(D_M(\text{MLP}(R_M(R_A(\mathbf{X}_2^*))))).
\end{align}
In essence, the equations comprise numerous ``Reduce" and ``Distribute" operations. However, these can be efficiently implemented by combining the operations and  reusing the local path features. 

